An analysis of budgeted parallel search on conditional Galton-Watson trees

Recently Avis and Jordan have demonstrated the efficiency of a simple technique called budgeting for the parallelization of a number of tree search algorithms. The idea is to limit the amount of work that a processor performs before it terminates its search and returns any unexplored nodes to a master process. This limit is set by a critical budget parameter which determines the overhead of the process. In this paper we study the behaviour of the budget parameter on conditional Galton-Watson trees obtaining asymptotically tight bounds on this overhead. We present empirical results to show that this bound is surprisingly accurate in practice.

==> luc_defs.tex <==
%-----------ADAPTED BY LUC FROM MSSYMB.TEX----------------------
%
%  Stuff for P V E S R in ocm style
\catcode`\@=11
\font\elevenocm=dsrom10 at 11pt
\font\sevenocm=dsrom10 at 7pt
\font\fiveocm=dsrom10 at 5pt
\font\elevenocm=ocmr10 at 11pt
\font\sevenocm=ocmr7
\font\fiveocm=ocmr5
%\font\elevenocm=BroadwayEngravedBT-Regular at 12pt
%\font\sevenocm=BroadwayEngravedBT-Regular at 9pt
%\font\fiveocm=BroadwayEngravedBT-Regular at 7pt
%
%\font\elevenocm=GoudyHandtooledBT-Regular at 10pt
%\font\tifont=GoudyHandtooledBT-Regular at 12pt
%\font\sevenocm=GoudyHandtooledBT-Regular at 8pt
%\font\fiveocm=GoudyHandtooledBT-Regular at 7pt
%
\newfam\ocmfam
\textfont\ocmfam=\elevenocm  \scriptfont\ocmfam=\sevenocm
  \scriptscriptfont\ocmfam=\fiveocm
\def\ocm{\ifmmode\let\next\ocm@\else
 \def\next{\errmessage{Use \string\ocm\space only in math mode}}\fi\next}
\def\ocm@#1{{\ocm@@{#1}}}
\def\ocm@@#1{\fam\ocmfam#1}
\catcode`\@=12
%-----------END OF STUFF FROM MSSYMB.TEX-------------------


\def\1modd{1~\hbox{\rm mod}~d}
\def\frac#1#2{{#1\over#2}} 
\def\PROB{{\ocm P}}
\def\prob#1{{\ocm P}\left\{ #1 \right\}}
\def\expec#1{{\ocm E}\left\{ #1 \right\}}
\def\IND#1{{\ocm 1}_{{\left[ #1 \right]}}}
\def\ind#1{{\ocm 1}_{{ #1 }}}
\def\EXP{{\ocm E}}
\def\FR#1#2{\raise 3pt\hbox{$\scriptstyle #1$}\kern-2.1pt/\kern-2pt\lower1.8pt\hbox{$\scriptstyle #2$}}
\def\shat{{\ocm S}}
\def\Var{{\ocm V}}
\def\var#1{{\ocm V}\left\{ #1 \right\}}
% \def\RR{{\mathop{\rm I{\kern-1.60pt}R}}}
\def\RR{{\ocm R}}
\def\inv{{\rm inv}}
\def\sumin{\sum_{i=1}^n}
\def\as{{\rm a.s.\ }}
\def\ip{{\rm i.p.\ }}
\def\io{{\rm i.o.\ }}
\def\isdef{\buildrel {\rm def} \over =}
\def\stochle{\buildrel {\rm (st)} \over \le}
\def\square{{\vcenter{\vbox{\hrule height .4pt
  \hbox{\vrule width .4pt height 7pt \kern7pt
  \vrule width .4pt}
  \hrule height .4pt}}}}
\def\scriptf{{\cal F}}
\def\essinf{\mathop{\rm ess\,inf}}
\def\argmin{\mathop{\rm arg\,min}}
\def\esssup{\mathop{\rm ess\,sup}}
\def\sech{\mathop{\rm sech}\nolimits}
\def\sign{\mathop{\rm sign}\nolimits}
\def\cosech{\mathop{\rm cosech}\nolimits}
\def\GAMMA{\mathop\Gamma\nolimits}
\def\PSI{\mathop\Psi\nolimits}
\def\PSIPRIME{\mathop{\Psi'}\nolimits}
\def\tendsinlaw{\buildrel {\cal L} \over \to}
\def\distributedas{\buildrel {\cal L} \over =}
\def\inlaw{\buildrel {\cal L} \over =}
\def\ddx{ {\hbox{\rm d} \over \hbox{\rm dx}} }
\def\stirling{\abovewithdelims[]}
%
% Boxes.
%
% \mathbox{width}{height}{linethickness} 
%    draws an empty box, as a square, for use
%    at ends of proofs. This is standardized
%    in \square. Never forget the $...$
%
% \rightbox{.}{.}{.} draws the same on the right
% \leftbox
% \centerbox 
%     
%    are similar once again
%
% \emptybox{.}{.}{.} does the same in a text
%
% 
% \textbox{text}{width} 
%    puts the said text in a box of the given width.
%


\def\mathbox#1#2#3{{\vcenter{\vbox{\hrule height #3%
  \hbox{\vrule width #3 height #2 \kern#1%
  \vrule width #3}%
  \hrule height #3}}}}%
\def\square{{\vcenter{\vbox{\hrule height .4pt%
  \hbox{\vrule width .4pt height 7pt \kern7pt%
  \vrule width .4pt}%
  \hrule height .4pt}}}}%
\def\rightbox#1#2#3{\rightline{$\mathbox{#1}{#2}{#3}$}}%
\def\leftbox#1#2#3{\leftline{$\mathbox{#1}{#2}{#3}$}}%
\def\centerbox#1#2#3{\centerline{$\mathbox{#1}{#2}{#3}$}}%
\def\emptybox#1#2#3{{\vbox{\hrule height #3%
  \hbox{\vrule width #3 height #2 \kern#1%
  \vrule width #3}%
  \hrule height #3}}}%
\long\def\textbox#1{\hbox{\vrule\vbox{\hrule\vskip 3pt\hbox%
  {\hskip 3pt #1\hskip 3pt}\vskip 3pt\hrule}%
  \vrule}}%
\def\figure#1\par{%
   \medskip%
   \centerline{\vbox{\hrule width 3.5in}}\smallskip%
   \centerline{Put Figure {#1} about here.} \smallskip%
   \centerline{\vbox{\hrule width 3.5in}}%
   \medskip}%

%
% Table inserts
%

\def \tablerule{\noalign{\smallskip\hrule\smallskip}}
\def \tabletoprule{\noalign{\hrule\smallskip}}
\def \tablebottomrule{\noalign{\smallskip\hrule}}
%
%              %%%%%%%    %%%%%        %%%%%%    %%%%%   %     %
%              %      %  %             %     %  %     %   %   %
%              %      %  %             %     %  %     %    % %
%              %%%%%%%    %%%%%        %%%%%%   %     %     %
%              %               %       %     %  %     %    % %
%              %               %       %     %  %     %   %   %
%              %         %%%%%%        %%%%%%    %%%%%   %     %
%
%              By Jean Orloff
%              Comments & suggestions by e-mail: ORLOFF@surya11.cern.ch
%              No modification of this file allowed if not e-sent to me.
%
% A simple way to measure the size of encapsulated postscript figures
%   from inside TeX, and to use it for automatically formatting texts
%   with inserted figures. Works both under Plain TeX-based macros
%   (Phyzzx, Harvmac, Psizzl, ...) and LaTeX environment.
% Provides exactly the same result on any PostScript printer provided
%   the single instruction \psfor... is changed to fit the needs of the
%   particular dvi->ps translator used.
% History:
%   1.32: corrects \psfordvialw and adds .TEX to PSBOXALL(!)
%   1.31: adds \psfordvialw(?)
%   1.30: adds \splitfile & \joinfiles for multi-file management
%   1.24: fix error handling & add \psonlyboxes
%   1.23: adds \putsp@ce for OzTeX fix
%   1.22: makes \drawingBox \global for use in Phyzzx
%   1.21: accepts %%BoundingBox: (atend)
%   1.20: tries to add \psfordvitps for the TeXPS package.
%   1.10: adds \psforoztex, error handling...
%2345678 1 2345678 2 2345678 3 2345678 4 2345678 5 2345678 6 2345678 7 23456789
%
% Checking version no to avoid multiple loadings
\def\temp{1.32}
\let\tempp=\relax
\expandafter\ifx\csname psboxversion\endcsname\relax
  \message{PSBOX(\temp) loading}
\else
    \ifdim\temp cm>\psboxversion cm
      \message{PSBOX(\temp) loading}
    \else
      \message{PSBOX(\psboxversion) is already loaded: I won't load
        PSBOX(\temp)!}
      \let\temp=\psboxversion
      \let\tempp=\endinput
    \fi
\fi
\tempp
\let\psboxversion=\temp
\catcode`\@=11
% Every macro likes a little privacy...
%
% Some common defs
%
\def\execute#1{#1}% NOT stupid: cs in #1 are then identified BEFORE execution
\def\psm@keother#1{\catcode`#112\relax}% borrowed from latex
\def\executeinspecs#1{%
\execute{\begingroup\let\do\psm@keother\dospecials\catcode`\^^M=9#1\endgroup}}
%
%Trying to tame the variety of \special commands for Postscript: the
%  universal internal command \PSspeci@l##1##2 takes ##1 to be the
%  filename and ##2 to be the integer scale factor*1000 (as for usual
%   TeX \scale commands)
%
\def\psfortextures{%     For TeXtures on the Macintosh
%-----------------
\def\PSspeci@l##1##2{%
\special{illustration ##1\space scaled ##2}%
}}
%
\def\psfordvitops{%      For the DVItoPS converter on IBM mainframes
%----------------
\def\PSspeci@l##1##2{%
\special{dvitops: import ##1\space \the\drawingwd \the\drawinght}%
}}
%
\def\psfordvips{%      For DVIPS converter on VAX, UNIX and PC's
%--------------
\def\PSspeci@l##1##2{%
%    \special{/@scaleunit 1000 def}% never read dox without trying!
\d@my=0.1bp \d@mx=\drawingwd \divide\d@mx by\d@my%
\special{PSfile=##1\space llx=\psllx\space lly=\pslly\space%
urx=\psurx\space ury=\psury\space rwi=\number\d@mx}%
}}
%
\def\psforoztex{%        For the OzTeX shareware on the Macintosh
%--------------
\def\PSspeci@l##1##2{%
\special{##1 \space
      ##2 1000 div dup scale
      \putsp@ce{\number-\psllx} \putsp@ce{\number-\pslly} translate
}%
}}
\def\putsp@ce#1{#1 }
%
\def\psfordvitps{%       From the UNIX TeXPS package, vers.>3.12
%---------------
% Convert a dimension into the number \psn@sp (in scaled points)
\def\psdimt@n@sp##1{\d@mx=##1\relax\edef\psn@sp{\number\d@mx}}
\def\PSspeci@l##1##2{%
% psfig.psr contains the def of "startTexFig": if you can locate it
% and include the correct pathname, it should work
\special{dvitps: Include0 "psfig.psr"}% contains def of "startTexFig"
\psdimt@n@sp{\drawingwd}
\special{dvitps: Literal "\psn@sp\space"}
\psdimt@n@sp{\drawinght}
\special{dvitps: Literal "\psn@sp\space"}
\psdimt@n@sp{\psllx bp}
\special{dvitps: Literal "\psn@sp\space"}
\psdimt@n@sp{\pslly bp}
\special{dvitps: Literal "\psn@sp\space"}
\psdimt@n@sp{\psurx bp}
\special{dvitps: Literal "\psn@sp\space"}
\psdimt@n@sp{\psury bp}
\special{dvitps: Literal "\psn@sp\space startTexFig\space"}
\special{dvitps: Include1 "##1"}
\special{dvitps: Literal "endTexFig\space"}
}}
\def\psfordvialw{%   Try for dvialw, a UNIX public domain
%---------------
\def\PSspeci@l##1##2{
\special{language "PostScript",
position = "bottom left",
literal "  \psllx\space \pslly\space translate
  ##2 1000 div dup scale
  -\psllx\space -\pslly\space translate",
include "##1"}
}}
\def\psonlyboxes{%     Draft-like behaviour if none of the others works
%---------------
\def\PSspeci@l##1##2{%
\at(0cm;0cm){\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at(0cm;0cm){\hbox{(##1)}}\hss}
  }}}
}%
}
%
\def\psloc@lerr#1{%
\let\savedPSspeci@l=\PSspeci@l%
\def\PSspeci@l##1##2{%
\at(0cm;0cm){\boxit{\vbox to\drawinght
  {\vss
  \hbox to\drawingwd{\at(0cm;0cm){\hbox{(##1) #1}}\hss}
  }}}
\let\PSspeci@l=\savedPSspeci@l% restore normal output for other figs!
}%
}
%
%\def\psfor...  add your own!
%
%  \ReadPSize{PSfilename} reads the dimensions of a PostScript drawing
%      and stores it in \drawinght(wd)
\newread\pst@mpin
\newdimen\drawinght\newdimen\drawingwd
\newdimen\psxoffset\newdimen\psyoffset
\newbox\drawingBox
\newif\ifNotB@undingBox
\newhelp\PShelp{Proceed: you'll have a 5cm square blank box instead of
your graphics (Jean Orloff).}
\def\@mpty{}
\def\s@tsize#1 #2 #3 #4\@ndsize{
  \def\psllx{#1}\def\pslly{#2}%
  \def\psurx{#3}\def\psury{#4}%  needed by a crazyness of dvips!
  \ifx\psurx\@mpty\NotB@undingBoxtrue% this is not a valid one!
  \else
    \drawinght=#4bp\advance\drawinght by-#2bp
    \drawingwd=#3bp\advance\drawingwd by-#1bp
%  !Units related by crazy factors as bp/pt=72.27/72 should be BANNED!
  \fi
  }
\def\sc@nline#1:#2\@ndline{\edef\p@rameter{#1}\edef\v@lue{#2}}
\def\g@bblefirstblank#1#2:{\ifx#1 \else#1\fi#2}
\def\psm@keother#1{\catcode`#112\relax}% borrowed from latex
\def\execute#1{#1}% Seems stupid, but cs are identified BEFORE execution
{\catcode`\%=12
\xdef\B@undingBox{%%BoundingBox}
}   %% is not a true comment in PostScript, even if % is!
\def\ReadPSize#1{
 \edef\PSfilename{#1}
 \openin\pst@mpin=#1\relax
 \ifeof\pst@mpin \errhelp=\PShelp
   \errmessage{I haven't found your postscript file (\PSfilename)}
   \psloc@lerr{was not found}
   \s@tsize 0 0 142 142\@ndsize
   \closein\pst@mpin
 \else
   \immediate\write\psbj@inaux{#1,}
   \loop
     \executeinspecs{\catcode`\ =10\global\read\pst@mpin to\n@xtline}
     \ifeof\pst@mpin
       \errhelp=\PShelp
       \errmessage{(\PSfilename) is not an Encapsulated PostScript File:
           I could not find any \B@undingBox: line.}
       \edef\v@lue{0 0 142 142:}
       \psloc@lerr{is not an EPSFile}
       \NotB@undingBoxfalse
     \else
       \expandafter\sc@nline\n@xtline:\@ndline
       \ifx\p@rameter\B@undingBox\NotB@undingBoxfalse
         \edef\t@mp{%
           \expandafter\g@bblefirstblank\v@lue\space\space\space}
         \expandafter\s@tsize\t@mp\@ndsize
       \else\NotB@undingBoxtrue
       \fi
     \fi
   \ifNotB@undingBox\repeat
   \closein\pst@mpin
 \fi
\message{#1}
}
%
% \psboxto(xdim;ydim){psfilename}: you specify the dimensions and
%    TeX uniformly scales to fit the largest one. If xdim=0pt, the
%    scale is fully determined by ydim and vice versa.
%    Notice: psboxes are a real vboxes; couldn't take hbox otherwise all
%    indentation and all cr's would be interpreted as spaces (hugh!).
%
\newcount\xscale \newcount\yscale \newdimen\pscm\pscm=1cm
\newdimen\d@mx \newdimen\d@my
\newdimen\pswdincr \newdimen\pshtincr
\let\ps@nnotation=\relax
\def\psboxto(#1;#2)#3{\vbox{
   \ReadPSize{#3}
   \advance\drawingwd by\pswdincr
   \advance\drawinght by\pshtincr
   \divide\drawingwd by 1000
   \divide\drawinght by 1000
   \d@mx=#1
   \ifdim\d@mx=0pt\xscale=1000
         \else \xscale=\d@mx \divide \xscale by \drawingwd\fi
   \d@my=#2
   \ifdim\d@my=0pt\yscale=1000
         \else \yscale=\d@my \divide \yscale by \drawinght\fi
   \ifnum\yscale=1000
         \else\ifnum\xscale=1000\xscale=\yscale
                    \else\ifnum\yscale<\xscale\xscale=\yscale\fi
              \fi
   \fi
   \divide \psxoffset by 1000\multiply\psxoffset by \xscale
   \divide \psyoffset by 1000\multiply\psyoffset by \xscale
   \global\divide\pscm by 1000
   \global\multiply\pscm by\xscale
   \multiply\drawingwd by\xscale \multiply\drawinght by\xscale
   \ifdim\d@mx=0pt\d@mx=\drawingwd\fi
   \ifdim\d@my=0pt\d@my=\drawinght\fi
   \message{scaled \the\xscale}
 \hbox to\d@mx{\hss\vbox to\d@my{\vss
   \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
      \kern-\psyoffset
      \PSspeci@l{\PSfilename}{\the\xscale}
      \vss}\hss\ps@nnotation}
   \global\ht\drawingBox=\the\drawinght
   \global\wd\drawingBox=\the\drawingwd
   \baselineskip=0pt
   \copy\drawingBox
 \vss}\hss}
  \global\psxoffset=0pt
  \global\psyoffset=0pt
  \global\pswdincr=0pt
  \global\pshtincr=0pt % These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}
%
% \psboxscaled{scalefactor*1000}{PSfilename} allows to bypass the
%   rounding errors of TeX integer divisions for situations where the
%   TeX box should fit the original BoundingBox with a precision better
%   than 1/1000.
%
\def\psboxscaled#1#2{\vbox{
  \ReadPSize{#2}
  \xscale=#1
  \message{scaled \the\xscale}
  \advance\drawingwd by\pswdincr\advance\drawinght by\pshtincr
  \divide\drawingwd by 1000\multiply\drawingwd by\xscale
  \divide\drawinght by 1000\multiply\drawinght by\xscale
  \divide \psxoffset by 1000\multiply\psxoffset by \xscale
  \divide \psyoffset by 1000\multiply\psyoffset by \xscale
  \global\divide\pscm by 1000
  \global\multiply\pscm by\xscale
  \global\setbox\drawingBox=\hbox to 0pt{\kern\psxoffset\vbox to 0pt{
     \kern-\psyoffset
     \PSspeci@l{\PSfilename}{\the\xscale}
     \vss}\hss\ps@nnotation}
  \global\ht\drawingBox=\the\drawinght
  \global\wd\drawingBox=\the\drawingwd
  \baselineskip=0pt
  \copy\drawingBox
  \global\psxoffset=0pt
  \global\psyoffset=0pt
  \global\pswdincr=0pt
  \global\pshtincr=0pt % These are local to one figure
  \global\pscm=1cm
  \global\drawingwd=\drawingwd
  \global\drawinght=\drawinght
}}
%
%  \psbox{PSfilename} makes a TeX box having the minimal size to
%      enclose the picture
\def\psbox#1{\psboxscaled{1000}{#1}}
%
%
%  \joinfiles file1, file2, ...n \into joinedfilename .
%     makes one file out of many
%  \splitfile joinedfilename
%     the opposite
%
%\def\execute#1{#1}% NOT stupid: cs in #1 are then identified BEFORE execution
%\def\psm@keother#1{\catcode`#112\relax}% borrowed from latex
%\def\executeinspecs#1{%
%\execute{\begingroup\let\do\psm@keother\dospecials\catcode`\^^M=9#1\endgroup}}
%\newread\pst@mpin
\newif\ifn@teof\n@teoftrue
\newif\ifc@ntrolline
\newif\ifmatch
\newread\j@insplitin
\newwrite\j@insplitout
\newwrite\psbj@inaux
\immediate\openout\psbj@inaux=psbjoin.aux
\immediate\write\psbj@inaux{\string\joinfiles}
\immediate\write\psbj@inaux{\jobname,}
%
% We redefine input to keep track of the various files inputted
%
\immediate\let\oldinput=\input
\def\input#1 {
 \immediate\write\psbj@inaux{#1,}
 \oldinput #1 }
\def\empty{}
\def\setmatchif#1\contains#2{
  \def\match##1#2##2\endmatch{
    \def\tmp{##2}
    \ifx\empty\tmp
      \matchfalse
    \else
      \matchtrue
    \fi}
  \match#1#2\endmatch}
\def\warnopenout#1#2{
 \setmatchif{TrashMe,psbjoin.aux,psbjoint.tex}\contains{#2}
 \ifmatch
 \else
   \immediate\openin\pst@mpin=#2
   \ifeof\pst@mpin
     \else
     \errhelp{If the content of this file is so precious to you, abort (ie
press x or e) and rename it before retrying.}
     \errmessage{I'm just about to replace your file named #2}
   \fi
   \immediate\closein\pst@mpin
 \fi
 \message{#2}
 \immediate\openout#1=#2}
%  No comments allowed below: % will have an unusual catcode
{
\catcode`\%=12
\gdef\splitfile#1 {
 \immediate\openin\j@insplitin=#1
 \message{Splitting file #1 into:}
 \warnopenout\j@insplitout{TrashMe}
 \loop
   \ifeof\j@insplitin
     \immediate\closein\j@insplitin\n@teoffalse
   \else
     \n@teoftrue
     \executeinspecs{\global\read\j@insplitin to\spl@tinline\expandafter
       \ch@ckbeginnewfile\spl@tinline%Beginning-Of-File-Named:%\endcheck}
     \ifc@ntrolline
     \else
       \toks0=\expandafter{\spl@tinline}
       \immediate\write\j@insplitout{\the\toks0}
     \fi
   \fi
 \ifn@teof\repeat
 \immediate\closeout\j@insplitout}
\gdef\ch@ckbeginnewfile#1%Beginning-Of-File-Named:#2%#3\endcheck{
 \def\t@mp{#1}
 \ifx\empty\t@mp
   \def\t@mp{#3}
   \ifx\empty\t@mp
     \global\c@ntrollinefalse
   \else
     \immediate\closeout\j@insplitout
     \warnopenout\j@insplitout{#2}
     \global\c@ntrollinetrue
   \fi
 \else
   \global\c@ntrollinefalse
 \fi}
\gdef\joinfiles#1\into#2 {
 \message{Joining following files into}
 \warnopenout\j@insplitout{#2}
 \message{:}
 {
 \edef\w@##1{\immediate\write\j@insplitout{##1}}
 \w@{% This text was produced with psbox's \string\joinfiles.}
 \w@{% To decompose and tex it:}
 \w@{%-save this with a filename CONTAINING ONLY LETTERS and a .TEX}
 \w@{% extension (say, JOINTFIL.TEX), in some uncrowded directory;}
 \w@{%-make sure you can \string\input\space psbox.tex (version>=1.3);}
 \w@{%-tex JOINTFIL.TEX using Plain, or LaTeX, or whatever is needed by}
 \w@{% the first part in the joining (after splitting JOINTFIL.TEX into}
 \w@{% it's constituents, TeX will try to process it as it stands).}
 \w@{\string\input\space psbox.tex}
 \w@{\string\splitfile{\string\jobname}}
 }
 \tre@tfilelist#1, \endtre@t
 \immediate\closeout\j@insplitout}
\gdef\tre@tfilelist#1, #2\endtre@t{
 \def\t@mp{#1}
 \ifx\empty\t@mp
   \else
   \llj@in{#1}
   \tre@tfilelist#2, \endtre@t
 \fi}
\gdef\llj@in#1{
 \immediate\openin\j@insplitin=#1
 \ifeof\j@insplitin
   \errmessage{I couldn't find file #1.}
   \else
   \message{#1}
   \toks0={%Beginning-Of-File-Named:#1}
   \immediate\write\j@insplitout{\the\toks0}
   \executeinspecs{\global\read\j@insplitin to\oldj@ininline}
   \loop
     \ifeof\j@insplitin\immediate\closein\j@insplitin\n@teoffalse
       \else\n@teoftrue
       \executeinspecs{\global\read\j@insplitin to\j@ininline}
       \toks0=\expandafter{\oldj@ininline}
       \let\oldj@ininline=\j@ininline
       \immediate\write\j@insplitout{\the\toks0}
     \fi
   \ifn@teof
   \repeat
   \immediate\closein\j@insplitin
 \fi}
}
% To be put at the end of a file, for making an tar-like file containing
%   everything it used.
\def\autojoin{
 \immediate\write\psbj@inaux{\string\into\space psbjoint.tex}
 \immediate\closeout\psbj@inaux
 \input psbjoin.aux
}
%
%  Annotations & Captions etc...
%
%
% \centinsert{anybox} is just a centered \midinsert, but is included as
%    people barely use the original inserts from TeX.
%
\def\centinsert#1{\midinsert\line{\hss#1\hss}\endinsert}
\def\psannotate#1#2{\vbox{
  \def\ps@nnotation{#2\global\let\ps@nnotation=\relax}#1}}
\def\pscaption#1#2{\vbox{
   \setbox\drawingBox=#1
   \copy\drawingBox
   \vskip\baselineskip
   \vbox{\hsize=\wd\drawingBox\setbox0=\hbox{#2}
     \ifdim\wd0>\hsize
       \noindent\unhbox0\tolerance=5000
    \else\centerline{\box0}
    \fi
}}}
% for compatibility with older versions, but \psfig is a bad name!
%\def\psfig#1#2#3{\pscaption{\psannotate{#1}{#2}}{#3}}
%\def\psfigurebox#1#2#3{\pscaption{\psannotate{\psbox{#1}}{#2}}{#3}}
%
% \at(#1;#2)#3 puts #3 at #1-higher and #2-right of the current
%    position without moving it (to be used in annotations).
\def\at(#1;#2)#3{\setbox0=\hbox{#3}\ht0=0pt\dp0=0pt
  \rlap{\kern#1\vbox to0pt{\kern-#2\box0\vss}}}
%
% \gridfill(ht;wd) makes a 1cm*1cm grid of ht by wd whose lower-left
%   corner is the current point
\newdimen\gridht \newdimen\gridwd
\def\gridfill(#1;#2){
  \setbox0=\hbox to 1\pscm
  {\vrule height1\pscm width.4pt\leaders\hrule\hfill}
  \gridht=#1
  \divide\gridht by \ht0
  \multiply\gridht by \ht0
  \gridwd=#2
  \divide\gridwd by \wd0
  \multiply\gridwd by \wd0
  \advance \gridwd by \wd0
  \vbox to \gridht{\leaders\hbox to\gridwd{\leaders\box0\hfill}\vfill}}
%
% Useful to measure where to put annotations
\def\fillinggrid{\at(0cm;0cm){\vbox{
  \gridfill(\drawinght;\drawingwd)}}}
%
% \textleftof\anybox: Sample text\endtext
%   inserts "Sample text" on the left of \anybox ie \vbox, \psbox.
%   \textrightof is the symmetric (not documented, too uggly)
% Welcome any suggestion about clean wraparound macros from
%   TeXhackers reading this
%
\def\textleftof#1:{
  \setbox1=#1
  \setbox0=\vbox\bgroup
    \advance\hsize by -\wd1 \advance\hsize by -2em}
\def\textrightof#1:{
  \setbox0=#1
  \setbox1=\vbox\bgroup
    \advance\hsize by -\wd0 \advance\hsize by -2em}
\def\endtext{
  \egroup
  \hbox to \hsize{\valign{\vfil##\vfil\cr%
\box0\cr%
\noalign{\hss}\box1\cr}}}
%
% \frameit{\thick}{\skip}{\anybox}
%    draws with thickness \thick a box around \anybox, leaving \skip of
%    blank around it. eg \frameit{0.5pt}{1pt}{\hbox{hello}}
% \boxit{\anybox} is a shortcut.
\def\frameit#1#2#3{\hbox{\vrule width#1\vbox{
  \hrule height#1\vskip#2\hbox{\hskip#2\vbox{#3}\hskip#2}%
        \vskip#2\hrule height#1}\vrule width#1}}
\def\boxit#1{\frameit{0.4pt}{0pt}{#1}}
% 

\newcount\figurenumber
\figurenumber=0



\outer\def\psfigure#1#2%
{\par
\medskip
\vbox{\baselineskip=10.8pt%
\global\advance\figurenumber by 1
$$\pscaption{\psbox{#1}}
{\rm%
{\bf Figure \the\figurenumber.\enspace}
#2}$$
\par\medskip
}
}

%
\catcode`\@=12 % cs containing @ are unreachable
%
% CUSTOMIZE YOUR DEFAULT DRIVER:
%    Uncomment the line corresponding to your TeX system:
%\psfortextures%     For TeXtures on the Macintosh
%\psforoztex   %     For OzTeX shareware on the Macintosh
%\psfordvitops %     For the DVItoPS converter for TeX on IBM mainframes
 \psfordvips   %     For DVIPS converter on VAX and UNIX
%\psfordvitps  %     For dvitps from TeXPS package under UNIX
%\psfordvialw  %     For dvialw, UNIX public domain
%\psonlyboxes  %     Blank Boxes (when all else fails).

\catcode`@=11 %borrow private macros of PLAIN, with care
\newskip\ttglue
\def\twelvepoint{%
\font\sc=cmcsc10
% \font\tifont=cmss12
\font\twelverm=cmr10
\font\twelvei=cmmi10
\font\twelvebi=cmmib10

\font\twelveex=cmex10
\font\twelvesy=cmsy10
% \font\twelvess=cmss12
% \font\twelvessbf=cmssbx10 at 12pt
\font\twelvebf=cmbx10
\font\twelvett=cmtt10
\font\twelvesl=cmsl10
\font\twelvesc=cmcsc10
\font\twelveit=cmti10
\font\twelveu=cmu10
% cmbx12.pfa cmbx7.pfa cmbx9.pfa cmcbx12.pfa cmcbx7.pfa cmcbx9.pfa cmccsc9.pfa cmcsc9.pfa cmcsl12.pfa cmcsl9.pfa cmcss12.pfa cmcss17.pfa cmcss9.pfa cmcssi12.pfa cmcssi17.pfa cmcssi9.pfa cmcti12.pfa cmcti7.pfa cmcti9.pfa cmctt12.pfa cmctt9.pfa cmcyr12.pfa cmcyr17.pfa cmcyr7.pfa cmcyr9.pfa cmmi12.pfa cmmi7.pfa cmmi9.pfa cmr12.pfa cmr17.pfa cmr7.pfa cmr9.pfa cmsl12.pfa cmsl9.pfa cmss12.pfa cmss17.pfa cmss9.pfa cmssi12.pfa cmssi17.pfa cmssi9.pfa cmsy7.pfa cmsy9.pfa cmtex9.pfa cmti12.pfa cmti7.pfa cmti9.pfa cmtt12.pfa cmtt9.pfa
\font\ninerm=cmr10 
\font\eightrm=cmr9 at 8pt
\font\eighti=cmmi9 at 8pt
\font\eightex=cmex10 at 8pt
\font\eightsy=cmsy9 at 8pt
% \font\eightss=cmss9 at 8pt
\font\eightbf=cmbx9 at 8pt
\font\eighttt=cmtt9 at 8pt
\font\eightsl=cmsl9 at 8pt
\font\eightit=cmti9 at 8pt
%\font\eightu=cmu10 at 9pt
\font\sixrm=cmr7
\font\sixi=cmmi7
\font\sixex=cmex10 at 7pt
\font\sixsy=cmsy7
% \font\sixss=cmss12 at 7pt
\font\sixbf=cmbx7
\font\sixtt=cmtt9 at 7pt
\font\sixsl=cmsl8 at 7pt
\font\sixit=cmti7
% \font\sixu=cmu10 at 6pt
\def\rm{\fam0\twelverm}%
  \textfont0=\twelverm \scriptfont0=\eightrm \scriptscriptfont0=\sixrm
  \textfont1=\twelvei \scriptfont1=\eighti \scriptscriptfont1=\sixi
  \textfont2=\twelvesy \scriptfont2=\eightsy \scriptscriptfont2=\sixsy
  \textfont3=\twelveex \scriptfont3=\eightex \scriptscriptfont3=\sixex
  \def\it{\fam\itfam\twelveit}%
  \textfont\itfam=\twelveit
  \def\sl{\fam\slfam\twelvesl}%
  \textfont\slfam=\twelvesl
  \def\bf{\fam\bffam\twelvebf}%
  \textfont\bffam=\twelvebf \scriptfont\bffam=\eightbf
   \scriptscriptfont\bffam=\sixbf
  \def\mit{\fam1}
  \def\oldstyle{\fam1\twelvei}
  \def\tt{\fam\ttfam\twelvett}%
  \textfont\ttfam=\twelvett
  \tt \ttglue=.5em plus.25em minus.15em
\hyphenchar\twelvett=-1 % inhibit hyphenation in typewriter type
  \baselineskip=12pt
  \normalbaselineskip=12pt
  \setbox\strutbox=\hbox{\vrule height8.5pt depth3.5pt width\z@}%
   % WAS for 12pt: 10-4, 14pt lead.
  \normalbaselines\rm}

\newdimen\pagewidth \newdimen\pageheight \newdimen\ruleht
 \hsize=38pc  \vsize=51pc  \maxdepth=2.2pt  \parindent=3pc
% BELOW ARE SPRINGER REQUESTS
% \hsize=4.5in \vsize=7.5in \parindent=20pt \maxdepth=2.2pt
\newdimen\HSIZE
\HSIZE=\hsize  % for double column stuff
% \hoffset=0.5in \voffset=0.7in
\pagewidth=\hsize \pageheight=\vsize \ruleht=.5pt
\abovedisplayskip=6pt plus 3pt minus 1pt
\belowdisplayskip=6pt plus 3pt minus 1pt
\abovedisplayshortskip=0pt plus 3pt
\belowdisplayshortskip=4pt plus 3pt
\overfullrule=0in  %no overfullrule
\newlinechar = `\|%
\outer\def\section#1\par{\vskip0pt plus.3\vsize\penalty-23
  \vskip0pt plus-.3\vsize\bigskip\medskip%\vskip\parskip
  \message{|#1|}\leftline{\bf#1}\nobreak\medskip}
\outer\def\subsection#1\par{\vskip0pt plus.3\vsize\penalty-18
  \vskip0pt plus-.3\vsize\bigskip%\vskip\parskip
  \message{|#1|}\noindent{\bf#1}}
\outer\def\proclaim #1. #2\par{\vskip0pt plus.3\vsize\penalty-15
  \vskip0pt plus-.3\vsize\bigskip\vskip\parskip
  \noindent{\sc#1.\enspace}{\sl#2}\par
  \ifdim\lastskip<\medskipamount \removelastskip\penalty13\bigskip\fi}
\outer\def\intermezzo#1{\vskip0pt plus.3\vsize\penalty-10
  \vskip0pt plus-.3\vsize\bigskip\vskip\parskip
  \noindent{\sc#1\enspace}}
\let\im\intermezzo
\outer\def\proof{\vskip0pt plus.3\vsize\penalty-15
  \vskip0pt plus-.3\vsize\bigskip\vskip\parskip
  \noindent{\sc Proof.\enspace}}
\outer\def\remark #1. #2\par{\vskip0pt plus.3\vsize\penalty-10
  \vskip0pt plus-.3\vsize\bigskip\medskip\vskip\parskip
  \noindent{\sc Remark #1.\enspace} #2\par
  \ifdim\lastskip<\medskipamount \removelastskip\penalty13\medskip\fi}
\def\title#1#2#3{\begingroup\null\bigskip\bigskip\tifont\halign{\centerline{##}\cr
  #1\cr #2\cr #3\cr}\bigskip\endgroup}




\outer\def\proclaim #1. #2\par{\vskip0pt plus.1\vsize\penalty-15
  \vskip0pt plus-.1\vsize\bigskip\vskip\parskip
  \noindent{\sc#1.\enspace}{\sl#2}\par
  \ifdim\lastskip<\medskipamount \removelastskip\penalty5\bigskip\fi}
\outer\def\intermezzo#1{\vskip0pt plus.1\vsize\penalty-5
  \vskip0pt plus-.1\vsize\bigskip\vskip\parskip
  \noindent{\sc#1\enspace}}
\let\im\intermezzo
\outer\def\proof{\vskip0pt plus.1\vsize\penalty-10
  \vskip0pt plus-.1\vsize\bigskip\vskip\parskip
  \noindent{\sc Proof.\enspace}}
\outer\def\remark #1. #2\par{\vskip0pt plus.1\vsize\penalty-5
  \vskip0pt plus-.1\vsize\bigskip\medskip\vskip\parskip
  \noindent{\sc Remark #1.\enspace} #2\par
  \ifdim\lastskip<\medskipamount \removelastskip\penalty5\medskip\fi}
\outer\def\abstract{\vskip0pt plus.1\vsize\penalty-25
  \vskip0pt plus-.1\vsize\bigskip\vskip\parskip
  \noindent{\sc Abstract.\enspace}}
\outer\def\continue{\medskip\noindent}
\outer\def\begindisplay{\begingroup\vskip0pt plus.1\vsize\penalty-25
  \vskip0pt plus-.1\vsize\bigskip\vskip\parskip
  \noindent\obeylines}
\outer\def\enddisplay{\ifdim\lastskip<\medskipamount \removelastskip\penalty5\bigskip\fi
  \endgroup}
% \outer\def\begindisplay{\obeylines\startdisplay}
% {\obeylines\gdef\startdisplay#1
  % {\catcode`\^^M=5$$#1\halign\bgroup\indent##\hfil&&\qquad##\hfil\cr}}
% \outer\def\enddisplay{\crcr\egroup$$}
\let\begintable=\beginalgo
\let\endtable=\endalgo
\def\title#1#2#3{\begingroup\null\bigskip\bigskip\tifont\halign{\centerline{##}\cr
  #1\cr #2\cr #3\cr}\bigskip\endgroup}
\def\author{\halign{\hfil##\hfil&\hfil##\hfil&\hfil##\hfil\cr
				    David Avis &and& Luc Devroye \cr
                                     &&\cr
                                    Department of Intelligence Science and Technology&&School of Computer Science\cr
                                    Graduate School of Informatics, Kyoto University&&McGill University\cr
                                    Yoshida-Honmachi, Sakyo-ku&&3450 University Street\cr
                                    Kyoto 606-8501&&Montreal H3A 2K6\cr
                                    Japan&&Canada\cr
                                    avis@i.kyoto-u.ac.jp&&luc@cs.mcgill.ca\cr
				    &&\cr
				    &&\cr
				    &&\cr}}
\outer\def\keywords{\medskip\noindent{\sc Keywords and phrases.}\ }
\outer\def\ams{\medskip\noindent{\sc 1991 Mathematics Subject Classifications:\ }}
\outer\def\crcat{\medskip\noindent{\sc CR Categories:\ }}
\outer\def\endpage{{\nopagenumbers\vfill
  \hrule\smallskip\noindent\ninerm
  \normalbaselineskip=11pt
  \setbox\strutbox=\hbox{\vrule height7.9pt depth3.1pt width\z@}
  \normalbaselines
  Corresponding author's address: Luc Devroye, School of Computer Science, McGill University, 3480
  University Street, Montreal, Canada H3A 2K6.
  Electronic address: {\tt http://luc.devroye.org}, {lucdevroye@gmail.com}.
  The author's research was sponsored by NSERC Grant A3456.
  \eject}}
\outer\def\doublespacing{}
  %{\normalbaselineskip=16pt
  %\setbox\strutbox=\hbox{\vrule height11.3pt depth4.7pt width\z@}
  %\normalbaselines}
\outer\def\singlespacing{
  \normalbaselineskip=13pt
  \setbox\strutbox=\hbox{\vrule height9pt depth4pt width\z@}
  \normalbaselines}


\def\beginalgo{\begingroup\vskip0pt plus .1\vsize\penalty-18
  \vskip0pt plus-.1\vsize\medskip\vskip\parskip\tt}
\def\endalgo{\par\bigskip
  \ifdim\lastskip<\medskipamount \removelastskip\penalty5\medskip\fi
  \endgroup}




%%%%\twelvepoint  % really 10pt
\parskip=10pt
\baselineskip=14pt
\normalbaselineskip=14pt
\setbox\strutbox=\hbox{\vrule height10pt depth4pt width\z@}%
\normalbaselines
\raggedbottom




%\title{The communication complexity of conditional Galton-Watson trees}{}{}
%
%$$\hbox to \hsize{\hfill\vbox{
%\author}\hfill
%}$$
%  \bigskip
%
%\vfill
%
%
%\abstract
%
%\vfill
%
%
%\keywords
%Random Galton-Watson tree, probabilistic
%analysis of algorithms, branching process.
%\vfill
%\crcat
%3.74, 5.25, 5.5.
%\vfill
%\ams
%60J80, 60J85,60G99.
%
%\vfill
%\endpage
%\smallskip
%
%\vfill\eject


